Towards Unifying Evaluation of Counterfactual Explanations: Leveraging Large Language Models for Human-Centric Assessments

As machine learning models evolve, maintaining transparency demands more human-centric explainable AI techniques. Counterfactual explanations, with roots in human reasoning, identify the minimal input changes needed to obtain a given output and, hence, are crucial for supporting decision-making. Despite their importance, the evaluation of these explanations often lacks grounding in user studies and remains fragmented, with existing metrics not fully capturing human perspectives. To address this challenge, we developed a diverse set of 30 counterfactual scenarios and collected ratings across 8 evaluation metrics from 206 respondents. Subsequently, we fine-tuned different Large Language Models (LLMs) to predict average or individual human judgment across these metrics. Our methodology allowed LLMs to achieve an accuracy of up to 63% in zero-shot evaluations and 85% (over a 3-classes prediction) with fine-tuning across all metrics. The fine-tuned models predicting human ratings offer better comparability and scalability in evaluating different counterfactual explanation frameworks.

==> Tables/LinearRegressionCoefficients.tex <==
\begin{table*}[t]
\centering
\caption{Feature coefficients in Linear Regression model. predicting overall satisfaction} \label{tab:LRImportances}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Feasibility} & \textbf{Consistency} & \textbf{Complet.} & \textbf{Trust} & \textbf{Understand.} & \textbf{Fairness} & \textbf{Complexity} \\
\hline
1.758&  0.410&  0.888&  1.768& -0.370&  0.046&  0.320 \\
\hline
\end{tabular}

\end{table*}

==> Tables/descriptive_statistics.tex <==
\begin{table}[h]
\centering


\begin{tabular}{|c|c|c|c|c|}
\hline
& mean  & stdv & min   & max  \\
             \hline
Satisfaction & 3.02  & 1.11 & 1.4   & 5.21 \\
\hline
Feasibility  & 3.27  & 1.15 & 1.34  & 5.11 \\
\hline
Consistency  & 3.69  & 1.14 & 1.77  & 5.43 \\
\hline
Completen.   & 3.38  & 0.92 & 1.78  & 5.33 \\
\hline
Trust        & 3.16  & 1.15 & 1.42  & 5.32 \\
\hline
Understand.  & 4.82  & 0.51 & 3.92  & 5.58 \\
\hline
Fairness     & 3.89  & 0.97 & 1.61  & 5.42 \\
\hline
Complexity   & -0.26 & 0.39 & -1.03 & 0.84
\\ \hline
\end{tabular}
\caption{Summary table for metric statistics calculated by taking mean of each statistic calculated individually for each question. Coefficient of variance is N/A for Complexity, as its scale does not have a meaningful zero.}
\label{tab:descriptive_statistics}
\end{table}

==> Tables/metric_definitions.tex <==
\begin{table}[h]
%\centering
\caption{Definitions of the evaluation criteria provided to the respondents in the questionnaire}
\label{tab:metric_definitions}
\begin{tabular}{|l|p{5cm}|}
\hline
\textbf{Metric} & \textbf{Definition} \\
\\ \hline
        
        Overall satisfaction& This scenario effectively explains how to reach a different outcome
        
    \\ \hline
        
         Feasibility&  The actions suggested by the explanation are practical, realistic to implement and actionable
         
    \\ \hline
         Consistency&  All parts of the explanation are logically coherent and do not contradict each other
         
    \\ \hline
         
         Completeness&  The explanation is sufficient in explaining the outcome
         
    \\ \hline
         
         Trust&  I believe that the suggested changes would bring about the desired outcome
         
    \\ \hline

         Understandability&  I feel like I understood the phrasing of the explanation well
         
    \\ \hline
         
         Fairness&  The explanation is unbiased towards different user groups and does not operate on sensitive features
         
    \\ \hline
         
        Complexity&  The explanation has an appropriate level of detail and complexity - not too simple, yet not overly complex
        
    \\ \hline
\end{tabular}
\end{table}

==> Tables/metric_definitions_and_scale.tex <==
\begin{table}[]
\begin{tabular}{|l|p{5cm}|}
\hline
\textbf{Metric and scale}                                            & \textbf{Definition}                                                                                        \\ \hline
\begin{tabular}[c]{@{}l@{}}Overall satisfaction\\ 1...6\end{tabular} & This scenario effectively explains how to reach a different outcome                                        \\ \hline
\begin{tabular}[c]{@{}l@{}}Feasibility\\ 1...6\end{tabular}          & The actions suggested by the explanation are practical, realistic to implement and actionable              \\ \hline
\begin{tabular}[c]{@{}l@{}}Consistency\\ 1...6\end{tabular}          & All parts of the explanation are logically coherent and do not contradict each other                       \\ \hline
\begin{tabular}[c]{@{}l@{}}Completeness\\ 1...6\end{tabular}         & The explanation is sufficient in explaining the outcome                                                    \\ \hline
\begin{tabular}[c]{@{}l@{}}Trust\\ 1...6\end{tabular}                & I believe that the suggested changes would bring about the desired outcome                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}Understandability\\ 1...6\end{tabular}    & I feel like I understood the phrasing of the explanation well                                              \\ \hline
\begin{tabular}[c]{@{}l@{}}Fairness\\ 1...6\end{tabular}             & The explanation is unbiased towards different user groups and does not operate on sensitive features       \\ \hline
\begin{tabular}[c]{@{}l@{}}Complexity\\ -2...2\end{tabular}          & The explanation has an appropriate level of detail and complexity - not too simple, yet not overly complex \\ \hline
\end{tabular}
\end{table}
